Code to Comment Translation: A Comparative Study on Model Effectiveness & Errors

Automated source code summarization is a popular software engineering research topic wherein machine translation models are employed to "translate" code snippets into relevant natural language descriptions. Most evaluations of such models are conducted using automatic reference-based metrics. However, given the relatively large semantic gap between programming languages and natural language, we argue that this line of research would benefit from a qualitative investigation into the various error modes of current state-of-the-art models. Therefore, in this work, we perform both a quantitative and qualitative comparison of three recently proposed source code summarization models. In our quantitative evaluation, we compare the models based on the smoothed BLEU-4, METEOR, and ROUGE-L machine translation metrics, and in our qualitative evaluation, we perform a manual open-coding of the most common errors committed by the models when compared to ground truth captions. Our investigation reveals new insights into the relationship between metric-based performance and model prediction errors grounded in an empirically derived error taxonomy that can be used to drive future research efforts

==> category.tex <==
\begin{table}[htb]
    \centering
    \tiny
\begin{tabular}{p{.5cm}p{3.5cm}|p{10cm}}
\toprule
 \textbf{Index} &   \textbf{Name} & \textbf{Definition} \\
     \midrule       
      \multicolumn{3}{c}{\textbf{Missing Context}}  \\\hline
     1.1 &                                 Missing Code &  Missing attributes that refers to the context \\
     1.2 &                 Missing Database information & Missing DB attribute that refers to the context \\
     \midrule       
      \multicolumn{3}{c}{\textbf{Missing information}}  \\\hline                                            
     2.1 &                    Missing specific information &  Missing vital information \\
     2.2 &                    Missing task elaboration, &  Failed to provide detailed insight from the code and provided only method name or attribute based short summary \\
     2.3 &                Missing non-vital information &  Missing non vital information but could improve meaning \\
     2.4 &              Missing Web-related information &  Failed to mention web-related identifier \\
     2.5 &                Failed to mention identifiers &  Whenever variable/attributes name could not be resolved like left as ‘\}’ or used a generic attribute name as ‘var’ \\
     2.6 &                           Missing Identifier & Fails to capture the identifier/attribute in its entirety [Not even with a wrong identifier/generic attribute name like ‘var’] \\
     2.7 &                      Missing Data Structures &  Misses specific data structure related information like string/array. \\
     2.8 &                   Missing syntax information &  Whenever variable/attributes name could not be resolved like left as ‘\}’ or used a generic attribute name as ‘var’ \\
     2.9 &                            Missing exception &  Missed exception errors specifically \\
     2.10 &                          Missing conditional &   Missed branching information \\
     \midrule       
      \multicolumn{3}{c}{\textbf{Incorrect Semantic Information}}  \\\hline     
     3.1 &                Partial incorrect information & Semantically matches most of the information but misses partial information \\
     3.2 &           Semantically unrelated to the code &  Totally out of context from the code\\
     3.3 &                    Algorithmically incorrect &  When it conveys different meaning than the code algorithm \\
     \midrule       
      \multicolumn{3}{c}{\textbf{Incorrect construction}}  \\\hline
     4.1 &               Incorrect identifier/attribute &  Successfully identified a variable or identifier past its generic appearance (like not just saying a ‘var’) but incorrectly attributes it \\
     4.2 &                          Incomplete sentence &  Whenever the predicted comment is grammatically incomplete \\
     4.3 &                                   Repetition &  Whenever there is a 2-3 repetition of a word or sub part of a sentence \\
     4.4 &                         Repetition [extreme] & Whenever there is greater than 3 repetition of a word or sub part of a sentence \\
     4.5 &                  Focusing on the method name &  Whenever ‘Description of Method’ is specified only focusing on the method name which also captures the method functionality to a good extent \\
     4.6 &                                Grammar error &  Whenever a grammatical error is encountered in a predicted output \\
     \midrule       
      \multicolumn{3}{c}{\textbf{Over Generalization}}  \\\hline
     5.1 &                            Different Meaning &  When it conveys different meaning than the code algorithm \\
     5.2 &                    Algorithmically incorrect &  over generalizes to a point where it conveys different meaning or operation \\
     5.3 &                           Missing Formatting &  Whenever variable/attributes name could not be resolved like left as ‘\}’ or used a generic attribute name as ‘var’ \\
     5.4 &              Missing attribute specification &  Where it uses the generic names like var instead of using the specific attribute name \\
     \midrule       
      \multicolumn{3}{c}{\textbf{Consistant with ground truth}}  \\\hline
     6.1 &                           With specific info &  When the produced output is in compliance with the ground truth with specific important information \\
     6.2 &                        Without specific info &  When the produced output is in compliance with the ground truth without specific important information \\
     6.3 &              Improvement in Semantic Meaning &  When the produced output is in compliance with the ground truth and conveys more natural information extracted from the code for better understandability \\
     6.4 &                  With unnecessary info added &  When the produced output is in compliance with the ground truth but with added redundant information \\
     \midrule       
      \multicolumn{3}{c}{\textbf{Extraneous/Unnecessary Information Included}}  \\\hline
     7.1 &       Unnecessary data structure information &  Adds incorrect data structure related information like string/array. \\
     7.2 &                 Unnecessary file information &          Adds unnecessary file related information \\
     7.3 &            Unnecessary incorrect information &   Adds unnecessary incorrect information \\
\bottomrule
\end{tabular}
    \caption{Category definition}
    \label{tab:cat}
\end{table}


